DualEquiNet: A Dual-Space Hierarchical Equivariant Network for Large Biomolecules

Geometric graph neural networks (GNNs) that respect E(3) symmetries have achieved strong performance on small molecule modeling, but they face scalability and expressiveness challenges when applied to large biomolecules such as RNA and proteins. These systems require models that can simultaneously capture fine-grained atomic interactions, long-range dependencies across spatially distant components, and biologically relevant hierarchical structure, such as atoms forming residues, which in turn form higher-order domains. Existing geometric GNNs, which typically operate exclusively in either Euclidean or Spherical Harmonics space, are limited in their ability to capture both the fine-scale atomic details and the long-range, symmetry-aware dependencies required for modeling the multi-scale structure of large biomolecules. We introduce DualEquiNet, a Dual-Space Hierarchical Equivariant Network that constructs complementary representations in both Euclidean and Spherical Harmonics spaces to capture local geometry and global symmetry-aware features. DualEquiNet employs bidirectional cross-space message passing and a novel Cross-Space Interaction Pooling mechanism to hierarchically aggregate atomic features into biologically meaningful units, such as residues, enabling efficient and expressive multi-scale modeling for large biomolecular systems. DualEquiNet achieves state-of-the-art performance on multiple existing benchmarks for RNA property prediction and protein modeling, and outperforms prior methods on two newly introduced 3D structural benchmarks demonstrating its broad effectiveness across a range of large biomolecule modeling tasks.

==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

% \subsection{Notations}
\textbf{Notations}. Each molecule can be represented as a 3D geometric graph, $\mathcal{G} = \{H, \boldsymbol{X} \}$. $H$ contains node features across hierarchical scales, specifically atom-level (e.g. atomic number) and residue-level (e.g. nucleotide type in RNA), denoted by $H = \{ {H_{atom} \in \mathbb{R}^{N_{atom} \times F_{atom}}, H_{res} \in \mathbb{R}^{N_{res} \times F_{res}}}\}$, where $N_{atom}$ and $N_{res}$ are the number of atoms and residues (e.g. the nucleotides in RNA and amino acids in proteins), $F_{atom}$ and $F_{res}$ are the dimensions of atom and residue features. $\boldsymbol{X} \in \mathbb{R}^{N_{atom} \times 3}$ denotes the 3D coordinates of atoms. Here from initial $\mathcal{G}$, we aim to construct Euclidean space neighbors $\mathcal{N}_{eu}$ and spherical harmonics space neighbors $\mathcal{N}_{sh}$. 
We use uppercase bold letters to denote matrices and lowercase symbols to represent the corresponding vectors for a given node. For example, $h_i$ and $\boldsymbol{x}_i$, for node $i$. To distinguish between invariant and equivariant features, we use regular letters for invariant features (e.g., $h$) and bold symbols for equivariant features (e.g., $\boldsymbol{x}$).


\subsection{E(3)-Equivariance and Spherical Harmonics}
\textbf{E(3)-Equivariance and Spherical Harmonics}. Equivariance to Euclidean transformations is a desirable property in geometric learning tasks involving 3D molecular structures. Specifically, a function \( f: \mathcal{X} \rightarrow \mathcal{Y} \) is said to be \textit{equivariant} with respect to a group \( \mathfrak{G} \) (e.g., the Euclidean group \(\mathrm{E}(3)\)) if, for any transformation $\mathfrak{g} \in \mathfrak{G}$ and any input $\boldsymbol{x} \in \mathcal{X}$, there exists a corresponding transformation \( \mathfrak{g} \) acting on the output space such that
\begin{equation}
    f(\mathfrak{g} \cdot \boldsymbol{x}) = \mathfrak{g} \cdot f(\boldsymbol{x}).
\end{equation}
For \(\mathrm{E}(3)\), this means that if the input (e.g., atomic coordinates or features) is rotated, translated, or reflected, the output of the model transforms in a consistent and predictable manner. This property ensures that the model's predictions are physically meaningful and invariant to arbitrary choices of coordinate systems—a key requirement for tasks involving 3D biomolecular data.

To achieve rotational equivariance in 3D, spherical harmonics are commonly used to represent directional features on the unit sphere. Spherical harmonics form an orthonormal basis for square-integrable functions defined on the sphere and serve as the irreducible representations of the rotation group \(\mathrm{SO}(3)\). A key property of these representations is their equivariant transformation under rotations. For a unit direction vector \(\hat{\boldsymbol{x}}\) and a rotation matrix \(\mathbf{R} \), the spherical harmonics basis of degree \(l\) transforms according to:
\[
Y^{(l)}(\mathbf{R} \hat{\boldsymbol{x}}) = \mathcal{D}^{(l)}(\mathbf{R}) \, Y^{(l)}(\hat{\boldsymbol{x}}),
\]
where \(Y^{(l)}(\cdot)\) is the spherical harmonics of degree \(l\), and \(\mathcal{D}^{(l)}(\mathbf{R}) \in \mathbb{R}^{(2l+1) \times (2l+1)}\) is the Wigner \(D\)-matrix corresponding to rotation \(\mathbf{R}\). This property enables the construction of rotation-equivariant functions by combining SH features with these bases, making them particularly suitable for encoding angular dependencies in molecular systems. We introduce more background in Appendix~\ref{appen:exp_details}.





